Bio-inspired Adaptive Latching System for Towing and Guiding Power-less Floating Platforms with Autonomous Robotic Boats

Autonomous robotic boats are expected to perform several tasks: 1) navigate autonomously in water environments, such as the canals of Amsterdam; 2) perform individual task, such as water monitoring, transporting goods and people; 3) latch together to create floating infrastructure, such as bridges and markets. In this paper we present a novel bio-inspired robotic system for latching, towing and guiding a floating passive-power-less platform. The challenge is to design an adaptive latching mechanism, able to create a secure connection between the entities, easy to attach/detach, even if the boats are affected by water disturbances. But most important, the adaptive latching must be able to restricting the DoF (degrees of freedom) of the latched "dummy" platform. Since, the robotic boat may drive it in narrow water canals and must prevent it from drifting and hitting the wall. This novel adaptive latching mechanism is based on the ball and socket joint that allows rotation and free movements in two planes at the same time. It consists of two parts: the male part that includes a bearing stud (ball) integrated on the floating bin "dummy" and the female part located on the autonomous robotic boat. Which integrates an adaptive framed funnel to guide the male ball into an actuated receptor that traps the ball, creating the ball-socket joint between the boats. In this sense, the adaptive latching mechanism mimics squid's tentacles that can adjust the forces applied to a holding object restricting its degrees of freedom. Experimental results are presented from our swarm robotic boats integrating the adaptive latching system and performing the towing and guiding use cases.

==> guiding.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SECTION: GUIDING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%The roboat's MPC controller is set to drive the robot next to another within  

In order to latch the roboat to a dock or to another robotic boat, a guiding system has been developed. This $guiding$ controller is activated, overriding the $driving$ control system, when the boats are set to latch and the detected distance between them is less than $125mm$.% in the real scale. %In our scaled prototype (1:4) the $guiding$ controller is activated when the detected distance between the parts is less than $125mm$.


\subsection{Guiding to a dock}
On the docks there are passive elements with only a permanent magnet as device to help direct the roboat for latching. %active male located on the robot. 
%The process of latching two roboats is more complex than the latching to a dock but it is more flexible. 
In this configuration, the active element (on-board the roboat) activates its 3D magnetometer to find the position that leads to the passive element on the dock. To do so, the magnetometer is configured as follows: %the z axis is dismissed since the boat and the male pin are floating on the same water level (we assume that the generated waves can be overcome by the funnel).
The $x$ and $y$ axis corners of the magnetometer are pointing outwards so when reaching to the magnetic field of the permanent magnet in the passive part, the position is related to a 2D plane and corrections can be made by the guiding controller. 
In other words, it is able to know the position of the magnet, whether it is located on the left or right of the pin, see Figure \ref{ffigguiding}.

%the roboat integrates a laser ranger for estimating the distance between itself and the dock or another roboat, the sensor range is $0-40m$  and with an accuracy of $\pm25mm$.

\subsubsection{Magnetic field }
The magnetometer integrated in the system is the BNO055, 
able to detect the magnetic field strength vector (20Hz) in three axis of magnetic field sensing in micro Tesla ($\mu$T). 
%a 3 axis capable of detect $\mu$T (micro Tesla). %The detection of the magnetic field is non-linear, nevertheless, from the detected values it is possible to know the direction of the magnetic field. % and have a raw estimation of the distance. %, see Table \ref{tablemagnetometer}
The permanent magnet is a NdFeB magnet with magnetization N42, and strength of $7.7kg$ (approx. $75.5N$). Figure \ref{ffigmagnet} shows the relation between the distance in $mm$ and $inclination$ angle in degrees with respect to the intensity in $\mu$T.



%\begin{table}[h]
%	\centering
%	\caption{My caption}
%	\label{tablemagnetometer}
%	\begin{tabular}{|l|l|l|l|l|}
%		\hline
%		a & b & c & d & e \\ \hline
%		1 & 2 & 3 & 4 & 5 \\ \hline
%		1 & 2 & 3 & 4 & 5 \\ \hline
%		1 & 2 & 3 & 4 & 5 \\ \hline
%	\end{tabular}
%\end{table}


%The framework communicate the IMU (Inertial Measurement Unit) reading respect to the heading angle, so the roboats 
%In order to know the roboats angle to each other


\subsection{Guiding to a roboat }
In the roboat to roboat latching, both parts are active and can be powered. The female part activates its electromagnet (with similar characteristics as the permanent magnet with $\sim 75N$ strength), while the male part activates its 3 axis magnetometer. Analogous to the previous case, the magnetometer helps to infer the position, while the roboats communicate IMU (Inertial Measurement Unit) data, in specific their heading angle to keep the roboats parallel to each other when guiding, see Algorithm \ref{a1}.

% and the laser ranger helps to estimate the distance between the roboats and to keep them parallel to each other. %Moreover, to acurately calculate the position within them, the photodiodes detect the light and frequency emitted by the LEDs from the active female. This helps to corroborate the socket position and perform the latching. % by keeping the boat no more than . %estimate the distance. Since, the magnetometer response is non-linear and the photodiodes response is almost linear with the light intensity.

%\subsubsection{LED detection}
%Another sensor to improve the detection of direction and distance is an array of photodiodes located on the male mechanism that detects the light emited from a female mechanism only on roboats (not on the dock).

%The light intensity varies linearly with the distance and thefore the system can corroborate the position and angle between the roboats. 

%from one sensor to the other the distance and position between the boats.



%\begin{figure}[thpb]
%	\centering
%	\includegraphics[width=0.45\textwidth]{figures/light.jpg}
%	\caption{Voltage output from photodiode.}
%	\label{ffigvisual}
%\end{figure}



\begin{algorithm}
	\caption{Guiding algorithm }
	\label{a1}
	\begin{algorithmic} 

		\REQUIRE Magnetometer axis X and Y %, $LaserRanger_{distance}$ 
		\ENSURE Distance to dock or roboat $d \leq 125mm$
		%\STATE $Magnetometer \leftarrow X Y$

		\IF {$d \leq 125mm$ AND\\ $Magnetometer_{X Y}\geq Threshold(\mu T)$}
		\STATE MOVE TOWARDS THE MAGNETIC FIELD

		\ELSE

		\STATE FIND MAGNETIC FIELD

		\ENDIF

	\end{algorithmic}
\end{algorithm}

%\begin{algorithm}
%	\caption{Guiding roboat to roboat latching }
%	\label{a2}
%	\begin{algorithmic} 
	
%	\REQUIRE $Magnetometer$ $M_{X\&Y}$, $LaserRanger_{distance}$%, $Light_{intensity}$ 
%	\ENSURE Distance to roboat $d \leq 125mm$
%	\STATE $Magnetometer \leftarrow axis X Y$
%	\STATE $\alpha$ (angle between roboats)
	
%	\IF {$d \leq 125mm$ AND $M_{X\&Y}\geq100\mu T$ AND $\alpha\leq5^\circ$}
%	\STATE MOVE TOWARDS THE MAGNETIC FIELD
	
%	\ELSE
	
%	\STATE FIND MAGNETIC FIELD%ROTATE TO GUARANTIE AN ANGLE BETWEEN THE ROBOATS $\leq30^\circ$
%	\ENDIF
	
%\end{algorithmic}
%\end{algorithm}



\subsection{Roboats guiding dynamics}
%The external perimeter of the funnel determines the degree of misalignment that the bearing stud (male pin) can have in order to enter.  
The current robotic boat prototype have dimensions $1000mm \times 500mm \times 250mm$; the designed funnel cone $h=110mm$ and $r=40mm$ resulting in circular area of acceptance $A_{acceptance}=5026.55mm^2$, and the integrated bearing stud radio is $bs_r=9mm$. 
%, resulting in circular area of acceptance is $A_{acceptance}=5026.55mm^2$.  
%While, the integrated bearing stud is  radio $bs_r=9mm$. 

In this configuration, the funnel plays a couple of key roles: First, its to accept the bearing stud from the male pin even if it is misaligned. Second, its to enable restricted movement in 3D space to the parts once the latching is performed.

In this context, the funnel is able to compensate the errors from the guiding controller and the water disturbances when the bearing stud is entering the funnel.  
This means that the funnel compensates the magnetic guidance error on the $X$ axis and the difference in height of the waves between the parts on the $Y$ axis.

%In this framework, the maximal water disturbance is given by the size of the funnel. In the 1:1 roboat the funnel is capable of compensate waves up to $320mm$. 




==> model.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SECTION: MODEL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[b]
	\centering
	\includegraphics[width=0.4\textwidth]{figures/BasicMovement.jpg}
	
	\caption{The six basic movements of an omnidirectional ASV.}
	\label{ffigonmi}
\end{figure}



\begin{figure*}[h]
	\centering
	\includegraphics[width=0.99\textwidth]{figures/passiveactive.jpg}
	\caption{
		a) Passive male. % integrates a bearing stud on the front of the pin, a sealed permanent magnet and soft plastic as damping system. 
		b) Active male. % integrates a bearing stud on the front of the pin, a 3-axis magnetometer, an array of photodiodes and an electromagnet. 
		c) Female. %Passive female integrates of a funnel to guide the male ball into a receptor that traps the ball. This receptor integrates a "push - lock" mechanism with three arms that when closed forms the ball-socket. Also, in the central axis of the "push - lock" mechanism a permanent magnet is embedded. The active female %in addition integrates an array of LED’s on the contour of the funnel and 
		%instead of the permanent magnet integrates an electromagnet.  In addition a servomotor on the back of the mechanism is used as emergency unlock. %  and  to guide the active male.
		d) Push - lock mechanism. % closes the three arms when its central axis is push inside, and opens when it is pulled out. 
	}
	\label{ffigpassiveactive}
\end{figure*}


The aim of the roboat latching system is to latch robotic boats to the dock and to other roboats to create floating infrastructure. %, such as bridges, stage concerts and floating markets. 
Therefore, the system is required to latch fast, secure and efficiently, while overcoming water disturbances, misaligments and weight unbalances.


\subsection{Roboat model}
The roboat is expected to be a robotic boat in a rectangular base $4m\times2m$ with four thrusters in the middle of its edges. In this relationship the roboat is able to move forward, backward, sideways and able to rotate on its axis, fulfilling all movements to be an omnidirectional robotic boat, see Figure  \ref{ffigonmi}. %\cite{fossen:guidance}. 

%, see Figure \ref{ffigroboatmodelr}$a$. 
The thrusters in the middle of the longer edges are used for moving forward and backwards, both of them are pointing in the same direction, where $a$ is the distance between these transverse propellers. While, the thrusters on the shorter edges are used for rotating and to move sideways, denoted by $b$ the distance between the longitudinal propellers, see Figure \ref{ffigroboatmodelr}$a$. 



\subsection{Latching mechanism model}

The latching system is based on the spherical joint, enabling the latched roboats to rotate and move in the surge and sway directions. %(ball and socket) that allows rotation and free movement in two planes at the same time. 
Meaning that one entity integrates the $ball$ end-effector (male) and the other robot integrates the $socket$ (female), see Figure \ref{ffigroboatmodelr}$b$. However, the robotic boats integrate both of them on board so they can connect to multiple roboats, see Figure \ref{ffigroboatmodelr}$d,e,f$. Depending on the use case, the roboat is configured with the right elements for the task. For instance, the roboat may only include female parts to tow other boats and connect them to a  docking station. This specific use case is presented in the experiments Section \ref{sec:experiments}. % to show the results from the indoor swimming pool and outdoor test on the Charles river and Amsterdam canals. 

In this context, the latching system considers two cases: 1) When a roboat is latching to a dock and 2) when a roboat is connecting to another roboat(s).

It is important to define these cases, because when latching to a dock, we don't want that the components on the dock are required to be powered. We expect passive elements that don't require maintenance, neither connection for power in any mean. %It can be floating waiting for the component on the roboat to latch it. 
However, when putting together two roboats, both components can be powered for integrating sensors and actuators in order to improve stability of the latching of the two moving (floating) platforms.

In this framework, there are four possible setups:

\subsubsection{Passive ball (male)}
The male part consists of a ball on the front-edge, a central axis covered with a protection rubber integrating a neodinium permanet magnet in its body, see Figure \ref{ffigpassiveactive}$a$.

\subsubsection{Active ball (male)}
Similar to the passive male, but can be powered and instead of a permanent magnet, it integrates an electromagnet and a 3-axis magnetometer, %and an array of photodiodes surrounding  the body of the pin, 
see Figure \ref{ffigpassiveactive}$b$. 
In addition, this pin can be extended/contracted from a linear actuator.

%Since, the passive female integrates a permanent magnet. 
%On the active male, the 3-axis magnetometer is used to find the direction and estimate the distance of the connection.  The electromagnet is used for unlocking the "push - lock" mechanism and unlach, while  the photodiodes are used to find and estimate the distance of an active female (located only on the roboat)

\subsubsection{Passive socket (female)}
The female part consists of a funnel to guide the male ball into a receptor that traps the ball, creating the spherical joint between the parts, see Figure \ref{ffigpassiveactive}$c$. This receptor integrates a "push - lock" mechanism with three arms that when closed forms the ball-socket and when open releases the trapped bearing stud. Also, in the receptor a permanent magnet is integrated, see Figure \ref{ffigpassiveactive}$d$.

\subsubsection{Active socket (female)}
Since this socket can be powered, it is similar to the passive socket but instead of a permanent magnet, it integrates an electromagnet %, an array of LED's on the contour of the funnel 
and an emergency unlatch system with a servomotor that opens the socket and releases the male pin. %This is usefull so either part can realise the binding.% to guide the active male.









